ODM: A Text-Image Further Alignment Pre-training Approach for Scene Text Detection and Spotting

In recent years, text-image joint pre-training techniques have shown promising results in various tasks. However, in Optical Character Recognition (OCR) tasks, aligning text instances with their corresponding text regions in images poses a challenge, as it requires effective alignment between text and OCR-Text (referring to the text in images as OCR-Text to distinguish from the text in natural language) rather than a holistic understanding of the overall image content. In this paper, we propose a new pre-training method called OCR-Text Destylization Modeling (ODM) that transfers diverse styles of text found in images to a uniform style based on the text prompt. With ODM, we achieve better alignment between text and OCR-Text and enable pre-trained models to adapt to the complex and diverse styles of scene text detection and spotting tasks. Additionally, we have designed a new labeling generation method specifically for ODM and combined it with our proposed Text-Controller module to address the challenge of annotation costs in OCR tasks, allowing a larger amount of unlabeled data to participate in pre-training. Extensive experiments on multiple public datasets demonstrate that our method significantly improves performance and outperforms current pre-training methods in scene text detection and spotting tasks. Code is available at https://github.com/PriNing/ODM.

==> sec/6_fl.tex <==
\newpage
\newpage
\appendix
\section{Appendix}

\begin{figure*}[t]
 \centering
 \includegraphics[width=1.\linewidth]{pic/apd/real.png}
 \label{fig:short-c}
 \caption{Visualization results on real images by ODM. }
 \label{fig:MIM}
\end{figure*}

\begin{figure*}[t]
 \centering
 
 \includegraphics[width=1.\linewidth]{pic/apd/syn.png}
 \label{fig:short-c}
 \caption{Visualization results on SynthText images by ODM.}
 \label{fig:MIM}
\end{figure*}

\begin{figure*}[t]
 \centering
 
 \includegraphics[width=1.\linewidth]{pic/apd/art.png}
 \label{fig:short-c}
 \caption{Visualization results on Art images by ODM}
 \label{fig:MIM}
\end{figure*}


\begin{figure*}[t]
 \centering
 
 \includegraphics[width=1.\linewidth]{pic/apd/MIM.png}
 \label{fig:short-c}
 \caption{Two forms of MIM. (a) the Universal MIM Method, masking the Whole Image; (b) Improved version of MIM for scene text, only masking the text region.}
 \label{fig:MIM}
\end{figure*}

\begin{table*}
  \centering
  % \tiny
  \caption{{$\dagger$} represents the scores obtained after reproducing the model}
  \resizebox{1\textwidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    \multirow{1}{*}{Method} &\multirow{1}{*}{P} & \multirow{1}{*}{R} & \multirow{1}{*}{H} \\
    \midrule

    DBNet++\cite{2022dbnetpp}{$\dagger$} & 91.61 & 81.46 & 86.24  \\
    DBNet++\cite{2022dbnetpp} + MIM & 89.12 & 84.79 & 86.90  \\
    DBNet++\cite{2022dbnetpp} + MIM(Only Text) & 91.34 & 83.29 & 87.13  \\
    DBNet++\cite{2022dbnetpp} + MLM(oCLIP\cite{language})& 90.37 & 84.98 & 87.59  \\
    DBNet++ + ODM & \textbf{91.87} & \textbf{85.94} & \textbf{88.81}  \\   
    % $\varDelta$ &  &  & \textcolor{red}{+ 1.46} \\

    \bottomrule              
    \end{tabular}
  }
  \label{tab:weak}
\end{table*}

